A Compendium of Control-Oriented Models of Gas Processing Equipment Components

This work provides linear control-oriented state space models of gas flow through standard equipment, such as valves, compressors, manifolds and non-trivial pipe geometries. After presenting the catalog of components, we show how to interconnect them: we briefly recall the matrix methodology derived elsewhere, accompanied by a Matlab example for a gas loop; secondly for the same example we provide an alternative approach using Matlab's connect function. All the aforementioned models are suited to model-based MIMO control design tools as they are in state-space form and they can be physically parametrized. Conservation of mass is the source of the algebraic constraints in and is a property subsumed in these new models. This is characterized by model transfer function properties at frequency zero. Each of the component models is shown to posses this property.

==> pid/pgflibraryshapes.gates.pid.ISO14617.code.tex <==
% MIT License
%
% Copyright (c) 2018 Jelle Spijker
%
% Permission is hereby granted, free of charge, to any person obtaining a copy
% of this software and associated documentation files (the "Software"), to deal
% in the Software without restriction, including without limitation the rights
% to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
% copies of the Software, and to permit persons to whom the Software is
% furnished to do so, subject to the following conditions:
%
% The above copyright notice and this permission notice shall be included in all
% copies or substantial portions of the Software.
%
% THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
% IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
% FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
% AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
% LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
% OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE
% SOFTWARE.

\pgfdeclareshape{generic circle ISO14617}
{
 % This shape is a generic circle, to which you can add something to
 % the before background path using the key
 % /pgf/generic circle ISO14617/before background
 % When this key is invoked, the transformation matrix will have been
 % setup such that the circle's center is at the origin and that the
 % position \pgfpoint{1pt}{0pt} lies exactly on the top of the circle
 % (and, there, on the middle of the line).
 \inheritsavedanchors[from=circle pid]
 \inheritanchorborder[from=circle pid]
 \inheritanchor[from=circle pid]{north}
 \inheritanchor[from=circle pid]{north west}
 \inheritanchor[from=circle pid]{north east}
 \inheritanchor[from=circle pid]{center}
 \inheritanchor[from=circle pid]{west}
 \inheritanchor[from=circle pid]{east}
 \inheritanchor[from=circle pid]{south}
 \inheritanchor[from=circle pid]{south west}
 \inheritanchor[from=circle pid]{south east}
 \inheritanchor[from=circle pid]{input}
 \inheritanchor[from=circle pid]{output}
 \inheritbackgroundpath[from=circle pid]

 \beforebackgroundpath{
  {
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgftransformshift{}
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
     \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
     \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgftransformscale{\pgf@sys@tonumber{\pgfutil@tempdima}}
    \pgfkeysvalueof{/pgf/generic circle ISO14617/before background}
   }
 }
}

% Generic rectangle, based on a rectangle pid
\pgfdeclareshape{generic rectangle ISO14617}
{
 % This shape is a generic rectangle, to which you can add something to
 % the before background path using the key
 % /pgf/generic rectangle ISO14617/before background
 % When this key is invoked, the transformation matrix will have been
 % setup such that the center is at the tip of the diode. The
 % position \pgfpoint{1pt}{0pt} lies exactly on the top of the
 % (suggested) line before the diode.
 \inheritsavedanchors[from=rectangle pid]
 \inheritanchor[from=rectangle pid]{center}
 \inheritanchor[from=rectangle pid]{north}
 \inheritanchor[from=rectangle pid]{south}
 \inheritanchor[from=rectangle pid]{east}
 \inheritanchor[from=rectangle pid]{west}
 \inheritanchor[from=rectangle pid]{north east}
 \inheritanchor[from=rectangle pid]{north west}
 \inheritanchor[from=rectangle pid]{south east}
 \inheritanchor[from=rectangle pid]{south west}
 \inheritanchor[from=rectangle pid]{input}
 \inheritanchor[from=rectangle pid]{output}
 \inheritanchorborder[from=rectangle pid]
 \inheritbackgroundpath[from=rectangle pid]

 \beforebackgroundpath {
  \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/minimum height}}
  \pgftransformyscale{\pgf@sys@tonumber{\pgf@xa}/2}
  \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/minimum width}}
  \pgftransformxscale{\pgf@sys@tonumber{\pgf@ya}/2}
  \pgfkeysvalueof{/pgf/generic rectangle ISO14617/before background}%
 }
}

\pgfkeys{
 /pgf/generic circle ISO14617/before background/.initial=,
 /pgf/generic rectangle ISO14617/before background/.initial=,
}

% Boiler, steam generator shape
\pgfdeclareshape{2531 ISO14617}
{
 \inheritsavedanchors[from=rectangle]
 \inheritanchorborder[from=rectangle]
 \inheritanchor[from=rectangle]{north}
 \inheritanchor[from=rectangle]{north west}
 \inheritanchor[from=rectangle]{north east}
 \inheritanchor[from=rectangle]{center}
 \inheritanchor[from=rectangle]{west}
 \inheritanchor[from=rectangle]{east}
 \inheritanchor[from=rectangle]{mid}
 \inheritanchor[from=rectangle]{mid west}
 \inheritanchor[from=rectangle]{mid east}
 \inheritanchor[from=rectangle]{base}
 \inheritanchor[from=rectangle]{base west}
 \inheritanchor[from=rectangle]{base east}
 \inheritanchor[from=rectangle]{south}
 \inheritanchor[from=rectangle]{south west}
 \inheritanchor[from=rectangle]{south east}
 \inheritbackgroundpath[from=rectangle]
 \anchor{input}{
  \pgf@process{\northeast}%
  \pgf@ya=.25\pgf@y%
  \pgf@process{\southwest}%
  \pgf@y=-.5\pgf@y%
  \advance\pgf@y by \pgf@ya%
 }
 \anchor{output}{%
  \pgf@process{\southwest}%
  \pgf@ya=-.25\pgf@y%
  \pgf@process{\northeast}%
  \pgf@y=.5\pgf@y%
  \advance\pgf@y by \pgf@ya%
 }

 \beforebackgroundpath {
  \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/minimum height}}
  \pgftransformyscale{\pgf@sys@tonumber{\pgf@xa}/2}
  \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/minimum width}}
  \pgftransformxscale{\pgf@sys@tonumber{\pgf@ya}/2}
  \pgfsys@beginscope
  \pgfpathmoveto{\pgfqpoint{-1pt}{0.5pt}}
  \pgfpathlineto{\pgfpoint{1pt}{0.5pt}}
  \pgfusepath{draw}
  \pgfsys@endscope
 }
}

% Regenerative pre-heater
\pgfdeclareshape{2518 ISO14617}
{
 \inheritsavedanchors[from=rectangle]
 \inheritanchorborder[from=rectangle]
 \inheritanchor[from=rectangle]{north}
 \inheritanchor[from=rectangle]{north west}
 \inheritanchor[from=rectangle]{north east}
 \inheritanchor[from=rectangle]{center}
 \inheritanchor[from=rectangle]{west}
 \inheritanchor[from=rectangle]{east}
 \inheritanchor[from=rectangle]{mid}
 \inheritanchor[from=rectangle]{mid west}
 \inheritanchor[from=rectangle]{mid east}
 \inheritanchor[from=rectangle]{base}
 \inheritanchor[from=rectangle]{base west}
 \inheritanchor[from=rectangle]{base east}
 \inheritanchor[from=rectangle]{south}
 \inheritanchor[from=rectangle]{south west}
 \inheritanchor[from=rectangle]{south east}
 \inheritbackgroundpath[from=rectangle]
 \anchor{cold}{
  \pgf@process{\northeast}%
  \pgf@ya=1.8\pgf@y%
  \pgf@xa=.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }
 \anchor{hot}{
  \pgf@process{\northeast}%
  \pgf@ya=-1.8\pgf@y%
  \pgf@xa=-.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{hot out}{
  \pgf@process{\northeast}%
  \pgf@ya=-1.8\pgf@y%
  \pgf@xa=-2.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x.5\pgf@x%
 }

 \anchor{hot in}{
  \pgf@process{\northeast}%
  \pgf@ya=-1.8\pgf@y%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \advance\pgf@y by \pgf@ya%
  \pgf@y=.5\pgf@y%
 }

 \anchor{cold in}{
  \pgf@process{\northeast}%
  \pgf@ya=1.8\pgf@y%
  \pgf@xa=-1.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x.5\pgf@x%
 }

 \anchor{cold out}{
  \pgf@process{\northeast}%
  \pgf@ya=1.8\pgf@y%
  \pgf@xa=2.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x.5\pgf@x%
 }

 \beforebackgroundpath {
  \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/minimum height}}
  \pgftransformyscale{\pgf@sys@tonumber{\pgf@xa}/2}
  \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/minimum width}}
  \pgftransformxscale{\pgf@sys@tonumber{\pgf@ya}/2}
  \pgfsys@beginscope
  \pgfpathmoveto{\pgfqpoint{-0.5pt}{0.5pt}}
  \pgfpathlineto{\pgfpoint{0.5pt}{0.5pt}}
  \pgfpathlineto{\pgfpoint{0.5pt}{0.85pt}}
  \pgfpathlineto{\pgfpoint{-0.5pt}{0.85pt}}
  \pgfpathclose
  \pgfusepath{draw}
  \pgfpathmoveto{\pgfqpoint{-0.5pt}{-0.5pt}}
  \pgfpathlineto{\pgfpoint{0.5pt}{-0.5pt}}
  \pgfpathlineto{\pgfpoint{0.5pt}{-0.85pt}}
  \pgfpathlineto{\pgfpoint{-0.5pt}{-0.85pt}}
  \pgfpathclose
  \pgfusepath{draw}
  \pgfsys@endscope

  \pgftransformyscale{\pgf@sys@tonumber{\pgf@xa}/48}
  \pgfsys@beginscope
  \pgfpathcircle{\pgfpoint{0pt}{0pt}}{0.5pt}
  \pgfusepath{draw}
  \pgfpathmoveto{\pgfqpoint{0.5734064310022943pt}{0.4015035054457322pt}}
  \pgfpatharc{35}{-35}{0.7pt}
  \pgfusepath{draw}
  \pgfsys@endscope
 }
}

% Cooling tower
\pgfdeclareshape{2521 ISO14617}
{
 \inheritsavedanchors[from=rectangle]
 \inheritanchorborder[from=rectangle]
 \inheritanchor[from=rectangle]{north}
 \inheritanchor[from=rectangle]{north west}
 \inheritanchor[from=rectangle]{north east}
 \inheritanchor[from=rectangle]{center}
 \inheritanchor[from=rectangle]{west}
 \inheritanchor[from=rectangle]{east}
 \inheritanchor[from=rectangle]{mid}
 \inheritanchor[from=rectangle]{mid west}
 \inheritanchor[from=rectangle]{mid east}
 \inheritanchor[from=rectangle]{base}
 \inheritanchor[from=rectangle]{base west}
 \inheritanchor[from=rectangle]{base east}
 \inheritanchor[from=rectangle]{south}
 \inheritanchor[from=rectangle]{south west}
 \inheritanchor[from=rectangle]{south east}
 \anchor{input}{
  \pgf@process{\northeast}%
  \pgf@ya=.25\pgf@y%
  \pgf@process{\southwest}%
  \advance\pgf@y by \pgf@ya%
 }
 \anchor{output}{%
  \pgf@process{\northeast}%
  \pgf@ya=-1.75\pgf@y%
  \pgf@process{\southeast}%
  \advance\pgf@y by \pgf@ya%
 }

 \beforebackgroundpath {
  \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/minimum height}}
  \pgftransformyscale{\pgf@sys@tonumber{\pgf@xa}/2}
  \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/minimum width}}
  \pgftransformxscale{\pgf@sys@tonumber{\pgf@ya}/2}
  \pgfsys@beginscope
  \pgfpathmoveto{\pgfpoint{-1}{-0.5pt}}
  \pgfpathlineto{\pgfpoint{-0.5pt}{1pt}}
  \pgfpathlineto{\pgfpoint{0.5pt}{1pt}}
  \pgfpathlineto{\pgfpoint{1pt}{-0.5pt}}
  \pgfpathlineto{\pgfpoint{-1pt}{-0.5pt}}
  \pgfpathlineto{\pgfpoint{-1pt}{-1pt}}
  \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
  \pgfpathlineto{\pgfpoint{1pt}{-0.5pt}}
  \pgfusepath{draw}
  \pgfsys@endscope
 }
}

% Heat-exchanger with straight tubes (fixed-tube plates)
\pgfdeclareshape{heat exchanger long ISO14617}
{
 \inheritsavedanchors[from=rectangle]
 \inheritanchorborder[from=rectangle]
 \inheritanchor[from=rectangle]{north}
 \inheritanchor[from=rectangle]{north west}
 \inheritanchor[from=rectangle]{north east}
 \inheritanchor[from=rectangle]{center}
 \inheritanchor[from=rectangle]{west}
 \inheritanchor[from=rectangle]{east}
 \inheritanchor[from=rectangle]{mid}
 \inheritanchor[from=rectangle]{mid west}
 \inheritanchor[from=rectangle]{mid east}
 \inheritanchor[from=rectangle]{base}
 \inheritanchor[from=rectangle]{base west}
 \inheritanchor[from=rectangle]{base east}
 \inheritanchor[from=rectangle]{south}
 \inheritanchor[from=rectangle]{south west}
 \inheritanchor[from=rectangle]{south east}
 \inheritbackgroundpath[from=rectangle]

 \anchor{fluid top}{
  \pgf@process{\northeast}%
  \pgf@ya=2.5\pgf@y%
  \pgf@xa=.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }
 \anchor{fluid bottom}{
  \pgf@process{\northeast}%
  \pgf@ya=-2.5\pgf@y%
  \pgf@xa=-.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{refrigerant top}{
  \pgf@process{\northeast}%
  \pgf@ya=2.1875\pgf@y%
  \pgf@xa=.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{refrigerant top left}{
  \pgf@process{\northeast}%
  \pgf@ya=2.1875\pgf@y%
  \pgf@xa=-1.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }
 \anchor{refrigerant top right}{
  \pgf@process{\northeast}%
  \pgf@ya=2.1875\pgf@y%
  \pgf@xa=2.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{refrigerant bottom}{
  \pgf@process{\northeast}%
  \pgf@ya=-2.1875\pgf@y%
  \pgf@xa=-.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{refrigerant bottom left}{
  \pgf@process{\northeast}%
  \pgf@ya=-2.1875\pgf@y%
  \pgf@xa=-2.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{refrigerant bottom right}{
  \pgf@process{\northeast}%
  \pgf@ya=-2.1875\pgf@y%
  \pgf@xa=1.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{fluid top}{
  \pgf@process{\northeast}%
  \pgf@ya=1.5625\pgf@y%
  \pgf@xa=.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }
 \anchor{fluid top right}{
  \pgf@process{\northeast}%
  \pgf@ya=1.5625\pgf@y%
  \pgf@xa=2.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }
 \anchor{fluid top left}{
  \pgf@process{\northeast}%
  \pgf@ya=1.5625\pgf@y%
  \pgf@xa=-1.5\pgf@x%
  \pgf@process{\southwest}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \anchor{fluid bottom}{
  \pgf@process{\northeast}%
  \pgf@ya=-1.5625\pgf@y%
  \pgf@xa=-.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }
 \anchor{fluid bottom right}{
  \pgf@process{\northeast}%
  \pgf@ya=-1.5625\pgf@y%
  \pgf@xa=1.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }
 \anchor{fluid bottom left}{
  \pgf@process{\northeast}%
  \pgf@ya=-1.5625\pgf@y%
  \pgf@xa=-2.5\pgf@x%
  \pgf@process{\northeast}%
  \pgf@y.5\pgf@y%
  \pgf@x.5\pgf@x%
  \advance\pgf@y by \pgf@ya%
  \advance\pgf@x by \pgf@xa%
  \pgf@y=.5\pgf@y%
  \pgf@x=.5\pgf@x%
 }

 \beforebackgroundpath {
  \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/minimum height}}
  \pgftransformyscale{\pgf@sys@tonumber{\pgf@ya}/2}
  \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/minimum width}}
  \pgftransformxscale{\pgf@sys@tonumber{\pgf@xa}/4}
  \pgfsys@beginscope
  \pgfpathmoveto{\pgfpoint{1pt}{0.75pt}}
  \pgfpathlineto{\pgfpoint{-1pt}{0.75pt}}
  \pgfusepath{draw}
  \pgfpathmoveto{\pgfpoint{1pt}{-0.75pt}}
  \pgfpathlineto{\pgfpoint{-1pt}{-0.75pt}}
  \pgfusepath{draw}
  \pgfsys@endscope
  \pgfsys@beginscope
  \pgfkeysvalueof{/pgf/heat exchanger long ISO14617/before background}%
  \pgfsys@endscope
 }
}

\pgfkeys{
 /pgf/heat exchanger long ISO14617/before background/.initial=,
}
\endinput

==> pid/pgflibraryshapes.gates.pid.code.tex <==
% MIT License
%
% Copyright (c) 2018 Jelle Spijker
%
% Permission is hereby granted, free of charge, to any person obtaining a copy
% of this software and associated documentation files (the "Software"), to deal
% in the Software without restriction, including without limitation the rights
% to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
% copies of the Software, and to permit persons to whom the Software is
% furnished to do so, subject to the following conditions:
%
% The above copyright notice and this permission notice shall be included in all
% copies or substantial portions of the Software.
%
% THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
% IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
% FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
% AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
% LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
% OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE
% SOFTWARE.

%
% Base shapes
%
% These shapes are identical to the shapes without "pid", only an "input"
% and an "output" anchor have been added at the left and right end.
\pgfdeclareshape{rectangle pid}
{
 \inheritsavedanchors[from=rectangle]
 \inheritanchorborder[from=rectangle]
 \inheritanchor[from=rectangle]{north}
 \inheritanchor[from=rectangle]{north west}
 \inheritanchor[from=rectangle]{north east}
 \inheritanchor[from=rectangle]{center}
 \inheritanchor[from=rectangle]{west}
 \inheritanchor[from=rectangle]{east}
 \inheritanchor[from=rectangle]{mid}
 \inheritanchor[from=rectangle]{mid west}
 \inheritanchor[from=rectangle]{mid east}
 \inheritanchor[from=rectangle]{base}
 \inheritanchor[from=rectangle]{base west}
 \inheritanchor[from=rectangle]{base east}
 \inheritanchor[from=rectangle]{south}
 \inheritanchor[from=rectangle]{south west}
 \inheritanchor[from=rectangle]{south east}
 \inheritbackgroundpath[from=rectangle]
 \anchor{input}{
  \pgf@process{\northeast}%
  \pgf@ya=.5\pgf@y%
  \pgf@process{\southwest}%
  \pgf@y=.5\pgf@y%
  \advance\pgf@y by \pgf@ya%
 }
 \anchor{output}{%
  \pgf@process{\southwest}%
  \pgf@ya=.5\pgf@y%
  \pgf@process{\northeast}%
  \pgf@y=.5\pgf@y%
  \advance\pgf@y by \pgf@ya%
 }
}

\pgfdeclareshape{circle pid}
{
 \inheritsavedanchors[from=circle]
 \inheritanchorborder[from=circle]
 \inheritanchor[from=circle]{north}
 \inheritanchor[from=circle]{north west}
 \inheritanchor[from=circle]{north east}
 \inheritanchor[from=circle]{center}
 \inheritanchor[from=circle]{west}
 \inheritanchor[from=circle]{east}
 \inheritanchor[from=circle]{mid}
 \inheritanchor[from=circle]{mid west}
 \inheritanchor[from=circle]{mid east}
 \inheritanchor[from=circle]{base}
 \inheritanchor[from=circle]{base west}
 \inheritanchor[from=circle]{base east}
 \inheritanchor[from=circle]{south}
 \inheritanchor[from=circle]{south west}
 \inheritanchor[from=circle]{south east}
 \inheritbackgroundpath[from=circle]
 % New:
 \anchor{input}{\centerpoint\advance\pgf@x by-\radius}
 \anchor{output}{\centerpoint\advance\pgf@x by\radius}
}


% Flow direction indicator. This shape uses the current setting of
% the flow direction arrow tip for the arrow. The shape is a
% rectangle around the arrow tip.
\pgfdeclareshape{direction pid}
{
 \savedanchor\northeast{
  \pgf@x=0pt%
  % Height is given by minimum height/2
  \pgfmathsetlength{\pgf@y}{\pgfkeysvalueof{/pgf/minimum height}}%
  \pgf@y=.5\pgf@y
 }
 \savedanchor\southwest{
  % Left border is given by left extend
  \pgfarrowtotallength{\pgfkeysvalueof{/pgf/direction pid arrow}}%
  \pgf@x=-\pgf@x%
  % Height is given by minimum height/2
  \pgfmathsetlength{\pgf@y}{\pgfkeysvalueof{/pgf/minimum height}}%
  \pgf@y=-.5\pgf@y
 }

 \inheritanchor[from=rectangle pid]{center}
 \inheritanchor[from=rectangle pid]{north}
 \inheritanchor[from=rectangle pid]{south}
 \inheritanchor[from=rectangle pid]{east}
 \inheritanchor[from=rectangle pid]{west}
 \inheritanchor[from=rectangle pid]{north east}
 \inheritanchor[from=rectangle pid]{north west}
 \inheritanchor[from=rectangle pid]{south east}
 \inheritanchor[from=rectangle pid]{south west}
 \inheritanchor[from=rectangle pid]{input}
 \inheritanchor[from=rectangle pid]{output}
 \inheritanchorborder[from=rectangle pid]
 \nodeparts{}% no text

 \behindbackgroundpath{
  \pgf@process{\southwest}
  \pgf@xa=\pgf@x
  \pgf@process{\northeast}
  \pgf@xb=\pgf@x
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{0pt}}
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{0pt}}
  \pgfusepathqstroke
 }

 \beforebackgroundpath{
  {
    \pgfsys@beginscope
    \pgfarrowdraw{\pgfkeysvalueof{/pgf/direction pid arrow}}%
    \pgfsys@endscope
   }
 }
}

\pgfkeys{
 /pgf/direction pid arrow/.initial=direction pid,
}

% Special arrow for pid directions:
\pgfarrowsdeclare{direction pid}{direction pid}
{
 \pgfmathsetlength\pgfutil@tempdima{\pgfgetarrowoptions{direction pid}}%
 \pgfutil@tempdima=.5\pgfutil@tempdima
 \pgfarrowsleftextend{+-\pgfutil@tempdima}
 \pgfarrowsrightextend{+\pgfutil@tempdima}
}
{
 \pgfmathsetlength\pgfutil@tempdima{\pgfgetarrowoptions{direction pid}}%
 \pgfsetdash{}{+0pt}
 \pgfsetroundjoin
 \pgfpathmoveto{\pgfqpoint{-0.5\pgfutil@tempdima}{0.38268343237\pgfutil@tempdima}}
 \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
 \pgfpathlineto{\pgfqpoint{-0.5\pgfutil@tempdima}{-0.38268343237\pgfutil@tempdima}}
 \pgfpathclose
 \pgfusepathqfillstroke
}

\pgfsetarrowoptions{direction pid}{4pt}

\endinput

==> pid/tikzlibrarycircuits.pid.ISO14617.code.tex <==
% MIT License
%
% Copyright (c) 2018 Jelle Spijker
%
% Permission is hereby granted, free of charge, to any person obtaining a copy
% of this software and associated documentation files (the "Software"), to deal
% in the Software without restriction, including without limitation the rights
% to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
% copies of the Software, and to permit persons to whom the Software is
% furnished to do so, subject to the following conditions:
%
% The above copyright notice and this permission notice shall be included in all
% copies or substantial portions of the Software.
%
% THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
% IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
% FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
% AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
% LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
% OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE
% SOFTWARE.

\usetikzlibrary{circuits.pid}
\usetikzlibrary{arrows}
\usepgflibrary{shapes.gates.pid.ISO14617}

% When this lib is loaded, all symbols default to ISO14617
\tikzset{
 circuit pid ISO14617/.style=
  {
   circuit pid,
   set 2301 graphic = 2301 ISO14617 graphic,
   set 2302 graphic = 2302 ISO14617 graphic,
   set 2101 graphic = 2101 ISO14617 graphic,
   set 2102 graphic = 2102 ISO14617 graphic,
   set 2103 graphic = 2103 ISO14617 graphic,
   set 2104 graphic = 2104 ISO14617 graphic,
   set 2151 graphic = 2151 ISO14617 graphic,
   set 1011 graphic = 1011 ISO14617 graphic,
   set 1041 graphic = 1041 ISO14617 graphic,
   set 1021 graphic = 1021 ISO14617 graphic,
   set 1022 graphic = 1022 ISO14617 graphic,
   set 685 graphic = 685 ISO14617 graphic,
   set 301 graphic = 301 ISO14617 graphic,
   set 2061 graphic = 2061 ISO14617 graphic,
   set 2065 graphic = 2065 ISO14617 graphic,
   set 2501 graphic = 2501 ISO14617 graphic,
   set 2511 graphic = 2511 ISO14617 graphic,
   set 2602 graphic = 2602 ISO14617 graphic,
   set 2037 graphic = 2037 ISO14617 graphic,
   set 2541 graphic = 2541 ISO14617 graphic,
   set 2531 graphic = 2531 ISO14617 graphic,
   set 2551 graphic = 2551 ISO14617 graphic,
   set 2062 graphic = 2062 ISO14617 graphic,
   set 2002 graphic = 2002 ISO14617 graphic,
   set 2518 graphic = 2518 ISO14617 graphic,
   set 2521 graphic = 2521 ISO14617 graphic,
   set 2514 graphic = 2514 ISO14617 graphic,
   set 2672 graphic = 2672 ISO14617 graphic,
   set 3801 graphic = 3801 ISO14617 graphic,
   set 3830 graphic = 3830 ISO14617 graphic,
   set 3806 graphic = 3806 ISO14617 graphic,
   set 751 graphic = 751 ISO14617 graphic,
   set 2602-bag graphic = 2602-bag ISO14617 graphic,
   set branch graphic = branch ISO14617 graphic,
   set crossing graphic = crossing ISO14617 graphic,
   set reference graphic = reference ISO14617 graphic,
  }
}

% Branch
\tikzset{
 branch ISO14617 graphic/.style={
   circuit symbol filled,
   circuit symbol size=width .5 height .5,
   shape=circle pid,
   outer sep=.25\pgflinewidth
  }
}

% crossing
\tikzset{
 crossing ISO14617 graphic/.style={
   circuit symbol wires,
   circuit symbol size=width 1 height .1,
   shape=generic circle ISO14617,
   draw=none,
   fill=white,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0.0pt}{-1.0pt}}
     \pgfpathlineto{\pgfpoint{0.0pt}{1.0pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Liquid pump
\tikzset{2301 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic circle ISO14617,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0.0pt}{-1.0pt}}
     \pgfpathlineto{\pgfpoint{1.0pt}{0.0pt}}
     \pgfpathlineto{\pgfpoint{0.0pt}{1.0pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Gas pump
\tikzset{2302 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic circle ISO14617,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-0.6pt}{-0.8pt}}
     \pgfpathlineto{\pgfpoint{0.9pt}{-0.4pt}}
     \pgfusepathqstroke
     \pgfpathmoveto{\pgfpoint{-0.6pt}{0.8pt}}
     \pgfpathlineto{\pgfpoint{0.9pt}{0.4pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Two-way valve
\tikzset{2101 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{0.6pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-0.6pt}}
     \pgfpathclose
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{1pt}{0.6pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-0.6pt}}
     \pgfpathclose
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Angled Two-way valve
\tikzset{2102 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{1pt}{0.6pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-0.6pt}}
     \pgfpathclose
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{-0.6pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.6pt}{-1pt}}
     \pgfpathclose
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Three-way valve
\tikzset{2103 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{0.6pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-0.6pt}}
     \pgfpathclose
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{1pt}{0.6pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-0.6pt}}
     \pgfpathclose
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{-0.6pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.6pt}{-1pt}}
     \pgfpathclose
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Four-way valve
\tikzset{2104 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{0.6pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-0.6pt}}
     \pgfpathclose
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{1pt}{0.6pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-0.6pt}}
     \pgfpathclose
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{-0.6pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.6pt}{-1pt}}
     \pgfpathclose
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{-0.6pt}{1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.6pt}{1pt}}
     \pgfpathclose
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Two- or three-way damper
\tikzset{2151 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2 height 2,
   shape=generic rectangle ISO14617,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-0.8pt}{0.8pt}}
     \pgfpathlineto{\pgfpoint{-0.1pt}{0.1pt}}
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{0.8pt}{-0.8pt}}
     \pgfpathlineto{\pgfpoint{0.1pt}{-0.1pt}}
     \pgfusepath{draw}
     \pgfpathcircle{\pgfpoint{0pt}{0pt}}{0.1}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% measurement point
\tikzset{
 1011 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size=width .5 height .5,
   shape=circle pid,
   fill=white,
   outer sep=.25\pgflinewidth
  }
}

% Sensor
\tikzset{751 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 3 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-0.65pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{-0.65pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{0pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Information-processing function
\tikzset{1041 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.25 height 1.25,
   shape=generic circle ISO14617,
   transform shape,
  }
}

% Automatic operation of a final controlling element
\tikzset{1022 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.25 height 1.25,
   shape=generic circle ISO14617,
   transform shape,
  }
}

% Manual operation of a final controlling element
\tikzset{1021 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.25 height 1.25,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{1pt}{0pt}}
     \pgfpatharc{0}{-180}{1pt}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Manual actuator operated by turning
\tikzset{685 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.25 height 1.25,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{-0.5pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1.5pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Envelope (tank)
\tikzset{301 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   transform shape,
  }
}

% Container tank, cistern for atmospheric pressure
\tikzset{2061 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{1pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{1pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Open store
\tikzset{2065 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{1pt}}
     \pgfusepath{draw}
     % \pgfsetdash{{7pt}{1pt}{1pt}{1pt}{1pt}{1pt}{21pt}{1pt}{1pt}{1pt}{1pt}{1pt}{8pt}}{0}
     \pgfpathmoveto{\pgfpoint{-0.8pt}{-1pt}}
     \pgfpathlineto{\pgfpointadd{\pgfpoint{-0.8pt}{-1pt}}{\pgfpointpolar{56.52883529}{0.5pt}}}
     \pgfpathmoveto{\pgfpointadd{\pgfpoint{-0.8pt}{-1pt}}{\pgfpointpolar{56.52883529}{1.25pt}}}
     \pgfpathlineto{\pgfpointadd{\pgfpoint{-0.8pt}{-1pt}}{\pgfpointpolar{56.52883529}{1.5pt}}}
     % \pgfpathmoveto{\pgfpointpolar{45}{0.25pt}}
     % \pgfpathlineto{\pgfpointpolar{45}{0.25pt}}
     % \pgfpathmoveto{\pgfpointpolar{45}{0.25pt}}
     % \pgfpathlineto{\pgfpointpolar{45}{0.25pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Heating or cooling coil
\tikzset{2501 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.25 height 1.25,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0pt}{-1pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Heating or cooling coil
\tikzset{2501 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.25 height 1.25,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0pt}{-1pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Screen or filter element
\tikzset{2602 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.25 height 1.25,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-2pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-1.15pt}{0pt}}
     \pgfpathmoveto{\pgfpoint{-0.65pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.65pt}{0pt}}
     \pgfpathmoveto{\pgfpoint{1.15pt}{0pt}}
     \pgfpathlineto{\pgfpoint{2pt}{0pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Bag screen or filter element
\tikzset{2602-bag ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-0.6pt}{0pt}}
     \pgfpathmoveto{\pgfpoint{-0.4pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-0.25pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-0.25pt}{-0.25pt}}
     \pgfpathmoveto{\pgfpoint{-0.25pt}{-0.45pt}}
     \pgfpathlineto{\pgfpoint{-0.25pt}{-0.70pt}}
     \pgfpathmoveto{\pgfpoint{-0.25pt}{-0.90pt}}
     \pgfpathlineto{\pgfpoint{0.25pt}{-0.90pt}}
     \pgfpathmoveto{\pgfpoint{1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.6pt}{0pt}}
     \pgfpathmoveto{\pgfpoint{0.4pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.25pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.25pt}{-0.25pt}}
     \pgfpathmoveto{\pgfpoint{0.25pt}{-0.45pt}}
     \pgfpathlineto{\pgfpoint{0.25pt}{-0.70pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Spray nozzle
\tikzset{2037 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 0.75 height 0.75,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0pt}{1pt}}
     \pgfpathlineto{\pgfpoint{-0.75pt}{-1pt}}
     \pgfpathmoveto{\pgfpoint{0pt}{1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{-1pt}}
     \pgfpathmoveto{\pgfpoint{0pt}{1pt}}
     \pgfpathlineto{\pgfpoint{0.75pt}{-1pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Fired type
\tikzset{2541 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1 height 1,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
     \pgfpathmoveto{\pgfpoint{-0.55pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0.15pt}}
     \pgfpathlineto{\pgfpoint{0.55pt}{-1pt}}
     \pgfpathmoveto{\pgfpoint{-1.5pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{1.5pt}{-1pt}}
     \pgfusepathqstroke
    },
   transform shape,
  }
}

% Rotary mixing element
\tikzset{2672 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2 height 1,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{1pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Boiler, steam generator
\tikzset{2531 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=2531 ISO14617,
   transform shape,
  }
}

% Heat pump, refrigerator or freezer
\tikzset{2551 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic circle ISO14617,
   draw=none,
   /pgf/generic circle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-1pt}}
     \pgfpathclose
     \pgfusepathqstroke

     \pgfpathellipse{\pgfqpoint{-0.15pt}{0.5pt}}{\pgfqpoint{0.05pt}{0.25pt}}{\pgfqpoint{0.15pt}{0.05pt}}
     \pgfusepath{draw}
     \pgfpathmoveto{\pgfpoint{-0.3pt}{0.5pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0.5pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Pressure or vacuum vessel
\tikzset{2062 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-0.5pt}{1pt}}
     \pgfpatharc{90}{270}{0.5pt and 1pt}
     \pgfpathmoveto{\pgfpoint{0.5pt}{1pt}}
     \pgfpatharc{270}{90}{-0.5pt and -1pt}
     \pgfpathmoveto{\pgfpoint{-0.5pt}{1pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{1pt}}
     \pgfpathmoveto{\pgfpoint{-0.5pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{-1pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Conveyor
\tikzset{3801 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 10 height 2.5,
   shape=generic rectangle ISO14617,
   transform shape,
  }
}

% Feeding funnel, hopper
\tikzset{3806 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 2.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{1pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{-1pt}}
     \pgfpathmoveto{\pgfpoint{1pt}{1pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{-1pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Spring
\tikzset{2002 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 0.5 height 1.5,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0pt}{1pt}}
     \pgfpathlineto{\pgfpoint{1pt}{0.7pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{0.35pt}}
     \pgfpathlineto{\pgfpoint{1pt}{-0.35pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-0.7pt}}
     \pgfpathlineto{\pgfpoint{0pt}{-1pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Screw type
\tikzset{3830 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.5 height 1,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{-1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{1pt}{0pt}}
     \pgfpathmoveto{\pgfpoint{0.7pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.35pt}{1pt}}
     \pgfpathlineto{\pgfpoint{-0.35pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{-0.7pt}{0pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Regenerative pre-heater
\tikzset{2518 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 4,
   shape=2518 ISO14617,
   transform shape,
  }
}

% Cooling tower
\tikzset{2521 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 5 height 8,
   shape=2521 ISO14617,
   transform shape,
  }
}

% Heat-exchanger with straight tubes (fixed-tube plates)
\tikzset{2511 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2 height 4,
   shape=heat exchanger long ISO14617,
   /pgf/heat exchanger long ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0pt}{0.75pt}}
     \pgfpathlineto{\pgfpoint{0pt}{-0.75pt}}
     \pgfpathmoveto{\pgfpoint{-0.5pt}{0.75pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{-0.75pt}}
     \pgfpathmoveto{\pgfpoint{0.5pt}{0.75pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{-0.75pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Heat-exchanger with coil-shaped tubes
\tikzset{2514 ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 2.5 height 5,
   shape=heat exchanger long ISO14617,
   /pgf/heat exchanger long ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{0.5pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{0.125pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{0.25pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{0.375pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{0.5pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{0.625pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0.6875pt}}
     \pgfpathlineto{\pgfpoint{0pt}{0.71pt}}

     \pgfpathmoveto{\pgfpoint{0.5pt}{0pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{-0.125pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{-0.25pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{-0.375pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{-0.5pt}}
     \pgfpathlineto{\pgfpoint{-0.5pt}{-0.625pt}}
     \pgfpathlineto{\pgfpoint{0pt}{-0.6875pt}}
     \pgfpathlineto{\pgfpoint{0pt}{-0.71pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

% Reference arrow
\tikzset{reference ISO14617 graphic/.style={
   circuit symbol lines,
   circuit symbol size = width 1.5 height 1.25,
   shape=generic rectangle ISO14617,
   draw=none,
   /pgf/generic rectangle ISO14617/before background={
     \pgfpathmoveto{\pgfpoint{1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{1pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{0.5pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{0.5pt}}
     \pgfpathmoveto{\pgfpoint{1pt}{0pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{-1pt}}
     \pgfpathlineto{\pgfpoint{0.5pt}{-0.5pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{-0.5pt}}
     \pgfpathlineto{\pgfpoint{-1pt}{0.5pt}}
     \pgfusepath{draw}
    },
   transform shape,
  }
}

==> pid/tikzlibrarycircuits.pid.code.tex <==
% MIT License
%
% Copyright (c) 2018 Jelle Spijker
%
% Permission is hereby granted, free of charge, to any person obtaining a copy
% of this software and associated documentation files (the "Software"), to deal
% in the Software without restriction, including without limitation the rights
% to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
% copies of the Software, and to permit persons to whom the Software is
% furnished to do so, subject to the following conditions:
%
% The above copyright notice and this permission notice shall be included in all
% copies or substantial portions of the Software.
%
% THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
% IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
% FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
% AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
% LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
% OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE
% SOFTWARE.

\usepackage{siunitx}
\usepackage{ifthen}
\usepackage{xparse}

\usetikzlibrary{circuits}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{intersections}
\usepgflibrary{shapes.gates.pid}

% Setting up an pid circuit
\tikzset{
 circuit pid/.style={
   circuit,
   every circuit pid/.try
  }
}

% Symbols user-friendly aliases
\tikzset{
 pump/.style={2301={#1}},
 compressor/.style={2302={#1}},
 fan/.style={2302={#1}},
 valve/.style={2101={#1}},
 angled valve/.style={2102={#1}},
 three way valve/.style={2103={#1}},
 four way valve/.style={2104={#1}},
 damper/.style={2151={#1}},
 measurement point/.style={1011={#1}},
 measurement device/.style={1041={#1}},
 information-processing function/.style={1041={#1}},
 function/.style={1041={#1}},
 manual operation/.style={1021={#1}},
 automatic operation/.style={1022={#1}},
 turning actuator/.style={685={#1}},
 spring/.style={2002={#1}},
 envelope/.style={301={#1}},
 tank/.style={301={#1}},
 tank atmospheric pressure/.style={2061={#1}},
 open store/.style={2065={#1}},
 container/.style={2061={#1}},
 cistern/.style={2061={#1}},
 boiler/.style={2531={#1}},
 steam generator/.style={2531={#1}},
 heat pump/.style={2551={#1}},
 refrigerator/.style={2551={#1}},
 freezer/.style={2551={#1}},
 pressure vessel/.style={2062={#1}},
 vacuum vessel/.style={2062={#1}},
 regenerative pre-heater/.style={2518={#1}},
 straight tube heat exchanger/.style={2511={#1}},
 cooling tower/.style={2521={#1}},
 coil shaped heat exchanger/.style={2514={#1}},
 sensor/.style={751={#1}},
 conveyor/.style={3801={#1}},
 screw type/.style={3830={#1}},
 feeding funnel/.style={3806={#1}},
}

% Annotations user-friendly aliases
\tikzset{
 displacement/.style={2321},
 rotodynamic/.style={2322},
 centrifugal/.style={2322},
 non return/.style={2111},
 globe/.style={2121},
 gate/.style={2124},
 safety function/.style={2112},
 central control room/.style={1101},
 local control room/.style={1103},
 heating coil/.style={2501={#1}},
 cooling coil/.style={2501={#1}},
 screen element/.style={2602={#1}},
 filter element/.style={2602={#1}},
 rotary mixing element/.style={2672={#1}},
 bag filter element/.style={2602-bag={#1}},
 spray nozzle/.style={2037={#1}},
 fired type/.style={2541={#1}},
 quantity transition to higher/.style={130},
 quantity transition to lower/.style={131},
 quantity transition to higher and lower/.style={132},
 device for separating/.style={2601},
 device for mixing/.style={2671},
}

% Path style user-friendly aliases
\tikzset{
functional path/.style={431},
signal flow/.style={249},
analogue signal path/.style={234},
mechanical link/.style={402},
shaft/.style={402},
slope/.style={3061},
slope'/.style={3061'},
}

% The default symbols (you need to load a sublib to install the actual rendering).
\tikzset{
 circuit declare symbol = 2301, % Liquid pump
 circuit declare symbol = 2302, % Gas pump
 circuit declare symbol = 2101, % Two-way valve
 circuit declare symbol = 2102, % Angled two-way valve
 circuit declare symbol = 2103, % Three-way valve
 circuit declare symbol = 2104, % Four-way valve
 circuit declare symbol = 2151, % Two- or three-way damper
 circuit declare symbol = 1011, % measurement point
 circuit declare symbol = 1041, % Information-processing function
 circuit declare symbol = 1021, % Manual operation of a final controlling element
 circuit declare symbol = 1022, % Automatic operation of a final controlling element
 circuit declare symbol = 685, % Manual actuator operated by turning
 circuit declare symbol = 2002, % Spring
 circuit declare symbol = 301, % Envelope (tank)
 circuit declare symbol = 2061, % Container tank, cistern for atmospheric pressure
 circuit declare symbol = 2501, % Heating or cooling coil
 circuit declare symbol = 2602, % Screen or filter element
 circuit declare symbol = 2602-bag, % Bag screen or filter element
 circuit declare symbol = 2672, % Rotary mixing element
 circuit declare symbol = 2037, % Spray nozzle
 circuit declare symbol = 2541, % Fired type
 circuit declare symbol = 2531, % Boiler, steam generator
 circuit declare symbol = 2551, % Heat pump, refrigerator or freezer
 circuit declare symbol = 2062, % Pressure or vacuum vessel
 circuit declare symbol = 2518, % Regenerative pre-heater
 circuit declare symbol = 2511, % Heat-exchanger with straight tubes (fixed-tube plates)
 circuit declare symbol = 2514, % Heat-exchanger with coil-shaped tubes
 circuit declare symbol = 2521, % Cooling tower
 circuit declare symbol = 751, % Sensor
 circuit declare symbol = 3801, % Conveyor
 circuit declare symbol = 3830, % Screw type
 circuit declare symbol = 3806, % Feeding funnel, hopper
 circuit declare symbol = 2065, % Open store
 circuit declare symbol = flow direction,
 circuit declare symbol = flow direction',
 circuit declare symbol = branch,
 circuit declare symbol = crossing,
 circuit declare symbol = reference,
 set flow direction graphic  = flow direction pid graphic,
 set flow direction' graphic = flow direction' pid graphic,
}

% The default units
\tikzset{
 circuit declare unit={speed}{\si{\meter\per\second}},
 circuit declare unit={mass flow}{\si{\kilo\gram\per\second}},
 circuit declare unit={volume flow}{\si{\cubic\meter\per\second}},
}

% The direction and arrow settings
\tikzset{
 annotation arrow/.style = {
   /utils/exec={\pgfsetarrowoptions{direction pid}{.25*\the\tikzcircuitssizeunit+.2*\the\pgflinewidth}},
   >=direction pid
  }
}

\tikzset{
 % These styles should set the end-arrow.
 %
 % This arrow will generally be used to indicate flow directions in a circuit:
 flow direction arrow/.style = {
   /utils/exec={\pgfsetarrowoptions{direction pid}{1.3065*.5*\the\tikzcircuitssizeunit+1.3065*.3*\the\pgflinewidth}},
   >=direction pid, direction pid arrow = direction pid,
  }
}

\tikzset{
flow direction pid graphic/.style = {
  shape=direction pid,
  circuit symbol filled,
  flow direction arrow,
  minimum width  = .5*\the\tikzcircuitssizeunit+.3*\the\pgflinewidth,
  minimum height = .5*\the\tikzcircuitssizeunit+.3*\the\pgflinewidth,
  transform shape
 },
flow direction' pid graphic/.style = {
flow direction pid graphic,
rotate=180
}
}

% Process measure and control
\tikzset{
 measure/.style args={#1}{
   append after command={%
     \pgfextra
     \node[scale=0.35, anchor=south, yshift=-2*\the\pgflinewidth] at (\tikzlastnode) {#1};
     \tikz@after@path%
     \endpgfextra
    }
  },
 at/.style args={#1#2#3}{
   above=#2\tikzcircuitssizeunit of #1, #3,
   append after command={%
     \pgfextra{
      \draw (\tikzlastnode) to (#1);}
    }
  },
 with/.style args={#1#2#3#4}{
   append after command={%
     \pgfextra{
      \node[#1={name=\tikzlastnode-#1,#4}] at ([xshift=#2*\tikzcircuitssizeunit,yshift=#3*\tikzcircuitssizeunit]\tikzlastnode) {};}
    }
  }
}

\newif\ifshowid\showidfalse
\newif\ifshowidinv\showidinvfalse

\tikzset{
id/.store in=\flowid,
id=P001,
pos/.store in=\flowpos,
pos=0.5,
pos slope/.store in=\flowposslope,
pos slope=0.5,
/tikz/show/.is if=showid,
/tikz/show'/.is if=showidinv,
/tikz/show=false,
/tikz/show'=false,
flow path/.style={
  name path global=\fsid\flowid,
  /utils/exec=\csname tikz@options\endcsname,
  decoration={
    markings,
    path has corners,
    mark=at position \flowpos
    with {
      \ifshowid \node[flow direction={info sloped=\fsid\flowid}] {}; \else \node[flow direction] {}; \fi
      \ifshowidinv \node[flow direction={info sloped={[rotate=-180,label distance=.5\tikzcircuitssizeunit]\fsid\flowid}}] {}; \else \node[flow direction] {}; \fi}
   },
  postaction={decorate}
  },
 249/.style={ % Direction of propagation, energy, or signal flow (simplex)
   decoration={
     markings,
     path has corners,
     mark=at position \flowpos
     with {
     \draw[solid] (-0.25\tikzcircuitssizeunit,-0.35\tikzcircuitssizeunit) to (0.25\tikzcircuitssizeunit,0) to (-0.25\tikzcircuitssizeunit,0.35\tikzcircuitssizeunit);
     }
    },
   postaction={decorate}
  },
431/.style={ % Pure functional type
  decoration={
    markings,
    mark=between positions 0 and 1 step 0.2 with {
      \draw[solid] (-0.25\tikzcircuitssizeunit,-0.25\tikzcircuitssizeunit) to (0.25\tikzcircuitssizeunit,0.25\tikzcircuitssizeunit);
     }
   },
  postaction={decorate}
 },
234/.style={
  decoration={
    markings,
    mark=between positions 0.2 and 0.8 step 0.2 with {
      \draw[solid] (-0.25\tikzcircuitssizeunit,-0.25\tikzcircuitssizeunit) to (-0.25\tikzcircuitssizeunit,0.125\tikzcircuitssizeunit)
      arc (180:0:0.25\tikzcircuitssizeunit) to (0.25\tikzcircuitssizeunit,-0.25\tikzcircuitssizeunit);
     }
   },
  postaction={decorate}
 },
402/.style={ % Mechanical link, shaft
  double distance=2
 },
3061/.style={ % Slope
  decoration={
    markings,
    mark=at position \flowposslope with {
      \draw (-.5\tikzcircuitssizeunit,0.7\tikzcircuitssizeunit) to (-0.5\tikzcircuitssizeunit,0.2\tikzcircuitssizeunit)
      to (0.5\tikzcircuitssizeunit,0.2\tikzcircuitssizeunit) to (-.5\tikzcircuitssizeunit,0.7\tikzcircuitssizeunit);
     }
   },
  postaction={decorate}
 },
3061'/.style={ % Slope
decoration={
  markings,
  mark=at position \flowposslope with {
    \draw (.5\tikzcircuitssizeunit,0.7\tikzcircuitssizeunit) to (0.5\tikzcircuitssizeunit,0.2\tikzcircuitssizeunit)
    to (-.5\tikzcircuitssizeunit,0.2\tikzcircuitssizeunit) to (.5\tikzcircuitssizeunit,0.7\tikzcircuitssizeunit);
   }
 },
postaction={decorate}
},
}


% Annotations
\tikzset{
 circuit declare annotation={2321}{0pt} % Positive-displacement type
  {
   (\tikzlastnode.north) edge[-,line width=0.5pt,line to] (\tikzlastnode.south)
  },
 circuit declare annotation={2322}{0pt} % Rotodynamic type
  {
   (\tikzlastnode.west) edge[-.,line width=0.5pt,line to] (\tikzlastnode.east)
  },
 circuit declare annotation={2111}{0pt} % Non-return function Flow from left to right possible
  {
   ([yshift=-0.6\tikzcircuitssizeunit,xshift=0.2\tikzcircuitssizeunit]\tikzlastnode.north west) edge[-,line width=2pt,to path={arc (-360:0:1pt)}] ()
  },
 circuit declare annotation={1101}{0pt} % Primary location in a central control room
  {
   (\tikzlastnode.east) edge[-,line width=0.5pt,line to] (\tikzlastnode.west)
  },
 circuit declare annotation={1103}{0pt} % Primary location in a local control room
  {
   ([xshift=-\the\pgflinewidth]\tikzlastnode.east) edge[double, -,line width=0.5pt,line to] ([xshift=\the\pgflinewidth]\tikzlastnode.west)
  },
 circuit declare annotation={adjustable}{1.5\tikzcircuitssizeunit}
  {
   ([xshift=-0.25\tikzcircuitssizeunit,yshift=-0.25\tikzcircuitssizeunit]\tikzlastnode.south west) edge[line to] ([xshift=0.25\tikzcircuitssizeunit, yshift=0.25\tikzcircuitssizeunit]\tikzlastnode.north east)
  },
 circuit declare annotation={adjustable'}{1.5\tikzcircuitssizeunit}
  {
   ([xshift=-0.25\tikzcircuitssizeunit,yshift=0.25\tikzcircuitssizeunit]\tikzlastnode.north west) edge[line to] ([xshift=0.25\tikzcircuitssizeunit, yshift=-0.25\tikzcircuitssizeunit]\tikzlastnode.south east)
  },
 circuit declare annotation={130}{0pt} % Transition to a higher quantity level
  {
   [shift=(\tikzlastnode.center),xshift=0.3\tikzcircuitssizeunit, yshift=0.5\tikzcircuitssizeunit]
   (0, -0.25\tikzcircuitssizeunit) edge[line to] (0,0.5\tikzcircuitssizeunit)
  },
 circuit declare annotation={131}{0pt} % Transition to a lower quantity level
  {
   [shift=(\tikzlastnode.center),xshift=0.3\tikzcircuitssizeunit, yshift=0.5\tikzcircuitssizeunit]
   (0,0.5\tikzcircuitssizeunit) edge[line to] (0, -0.25\tikzcircuitssizeunit)
  },
 circuit declare annotation={132}{0pt} % Transition to a higher or lower quantity level
  {
   [shift=(\tikzlastnode.center),xshift=0.3\tikzcircuitssizeunit, yshift=0.5\tikzcircuitssizeunit]
   (0,0.5\tikzcircuitssizeunit) edge[<->,line to] (0, -0.25\tikzcircuitssizeunit)
  },
 circuit declare annotation={2112}{0pt} % Safety function
  {
   [shift=(\tikzlastnode.north east),xshift=-0.3\tikzcircuitssizeunit, yshift=-0.3\tikzcircuitssizeunit]
   (0,0) edge[-,line to] ([xshift=-0.3\tikzcircuitssizeunit, yshift=0.3\tikzcircuitssizeunit]\tikzlastnode.south east)
  },
 circuit declare annotation={2121}{0pt} % Globe type
  {
   ([xshift=2pt]\tikzlastnode.center) edge[-,line width=4pt,to path={arc (-360:0:2pt)}] ()
  },
 circuit declare annotation={light}{0pt} % N
  {
   ([xshift=-0.75\tikzcircuitssizeunit,yshift=1\tikzcircuitssizeunit]\tikzlastnode.north) edge[line to] ([xshift=-0.25\tikzcircuitssizeunit,yshift=0.1\tikzcircuitssizeunit]\tikzlastnode.north)
   ([xshift=-0.25\tikzcircuitssizeunit,yshift=1\tikzcircuitssizeunit]\tikzlastnode.north) edge[line to] ([xshift=0.25\tikzcircuitssizeunit,yshift=0.1\tikzcircuitssizeunit]\tikzlastnode.north)
  },
 circuit declare annotation={2601}{0pt} % N
  {
   ([xshift=-0.75\tikzcircuitssizeunit,yshift=0.75\tikzcircuitssizeunit]\tikzlastnode.center) edge[line to] ([xshift=0.75\tikzcircuitssizeunit,yshift=0.75\tikzcircuitssizeunit]\tikzlastnode.center)
   ([xshift=-0.25\tikzcircuitssizeunit,yshift=0.75\tikzcircuitssizeunit]\tikzlastnode.center) edge[line to] ([xshift=0.65\tikzcircuitssizeunit,yshift=0.35\tikzcircuitssizeunit]\tikzlastnode.center)
  },
  circuit declare annotation={2671}{0pt} % N
   {
    ([xshift=-0.75\tikzcircuitssizeunit,yshift=0.75\tikzcircuitssizeunit]\tikzlastnode.center) edge[line to] ([xshift=0.75\tikzcircuitssizeunit,yshift=0.75\tikzcircuitssizeunit]\tikzlastnode.center)
    ([xshift=0.25\tikzcircuitssizeunit,yshift=0.75\tikzcircuitssizeunit]\tikzlastnode.center) edge[-,line to] ([xshift=-0.65\tikzcircuitssizeunit,yshift=0.35\tikzcircuitssizeunit]\tikzlastnode.center)
   },
  circuit declare annotation={2124}{0pt} % Gate type
   {
    (\tikzlastnode.north) edge[-,line to] (\tikzlastnode.south)
   },
}

\makeatletter
% Helper command to get the current coordinates in a path
\newcommand\currentcoordinate{\the\tikz@lastxsaved,\the\tikz@lastysaved}

% Helper to place crossing
\newcommand{\crossings}[2]{
 \fill [name intersections={of=#1 and #2, name=i, total=\t}]
 \foreach \s in {1,...,\t}{(i-\s) node[crossing] {}};
}

% flow system environment
\pgfkeys{
 flow system/.is family, /flow system,
 fsdefault/.style =
  {color=black, id=0, line type=solid, line width=0.25mm},
 color/.estore in = \fscolor,
 id/.estore in = \fsid,
 id=,
 line type/.estore in = \fslinetype,
 line width/.estore in = \fslinewidth,
}

\NewDocumentEnvironment{flow system} { o }
{
 \pgfkeys{/flow system, fsdefault, #1}
 \begin{scope}[\fscolor, line width=\fslinewidth, \fslinetype]
  }
  {
 \end{scope}
}

% control system environment
\pgfkeys{
 control system/.is family, /control system,
 csdefault/.style =
  {color=black, id=0, line type=densely dashed, line width=0.15mm},
 color/.estore in = \cscolor,
 id/.estore in = \csid,
 id=,
 line type/.estore in = \cslinetype,
 line width/.estore in = \cslinewidth,
}

\NewDocumentEnvironment{control system} { o }
{
 \pgfkeys{/control system, csdefault, #1}
 \begin{scope}[\cscolor, line width=\cslinewidth, \cslinetype]
  }
  {
 \end{scope}
}

% complex device environment
\newif\ifshowcdlabel\showcdlabelfalse
\newif\ifshowcdborder\showcdborderfalse

\pgfkeys{
 complex device/.is family, /complex device,
 cddefault/.style =
  {name=device,xshift=0,yshift=0,rotate=0, border=5, border line type=dash dot, border line width=0.25mm, border color=black, scale=1},
 xshift/.estore in = \cdxshift,
 yshift/.estore in = \cdyshift,
 rotate/.estore in = \cdrotate,
 name/.estore in = \cdname,
 show label/.is if = showcdlabel,
 show border/.is if = showcdborder,
 border/.estore in = \cdborder,
 border line type/.estore in = \cdborderlinetype,
 border line width/.estore in = \cdborderlinewidth,
 border color/.estore in = \cdbordercolor,
 scale/.estore in = \cdborderscale,
}

\NewDocumentEnvironment{complex device} { o }
{
 \pgfkeys{/complex device, cddefault, #1}
 \begin{scope}[xshift=\cdxshift, yshift=\cdyshift, rotate=\cdrotate, local bounding box=\cdname, transform canvas={scale=\cdborderscale}]
  }
  {
  \ifshowcdborder \draw[\cdbordercolor, \cdborderlinetype, line width=\cdborderlinewidth] ([xshift=-\cdborder,yshift=\cdborder]\cdname.north west) rectangle ([xshift=\cdborder,yshift=-\cdborder]\cdname.south east); \fi
  \ifshowcdlabel \node at ([yshift=\cdborder+4]\cdname.north) {\cdname}; \fi
 \end{scope}
}
\makeatother

\endinput
